Simulating Geomagnetic Effects on Muons in Extensive Air Showers for the EUSO-SPB2 Mission

The Extreme Universe Space Observatory on a Super Pressure Balloon II (EUSO-SPB2) measured extensive air showers (EASs) from upward-going High Energy Cosmic Rays by flying a Cherenkov Telescope (CT) at 33 km altitude. The telescope could be tilted just above the Earth's limb, 5.8 degrees below horizontal, and 650 km away as viewed from the balloon. This configuration enables the detection of EASs that develop over a longer path length than downward-going showers. The lifetime of 100 GeV muons, as an example, corresponds to a path length of 620 km in Earth's upper atmosphere, where there is a decreased amount of energy lost due to atmospheric interactions (only approximately 40 MeV/km lost at 15 km altitude). In this configuration, muons can travel hundreds of kilometers while bending in Earth's geomagnetic field before they decay. These effects cause EASs to be more dense with muons at larger shower depths compared to the shower at Xmax, a result known as the muon tail. The objective of this simulation is to understand whether the CT on EUSO-SPB2 could measure the Cherenkov signal produced by the muon tail and observe the effects of the muons deflecting in Earth's geomagnetic field. We found that the timing and angular distributions of the Cherenkov signal allow the muon component to be separated from the main Cherenkov signal and we identified quantifiable effects of the muons deflecting in the geomagnetic field. However, at this time we are unable to simulate enough events to analyze the distribution of photons arriving in an area the size of the aperture of the CT. Thus, we cannot make conclusions about whether these effects can be seen by EUSO-SPB2.

==> JEM-EUSO_Authors_July2023.tex <==
{\Large\bf Full Authors list: The JEM-EUSO Collaboration\\}
%{\scriptsize (author-list as of July 1st, 2023)} \hspace{0.6cm}
%{\scriptsize (version  \today{} \currenttime{})}
%\vspace*{0.5cm}

\begin{sloppypar}
{\small \noindent
S.~Abe$^{fq}$, 
J.H.~Adams Jr.$^{pd}$, 
D.~Allard$^{cb}$,
P.~Alldredge$^{pd}$,
L.~Anchordoqui$^{pe}$,
A.~Anzalone$^{eh,ed}$, 
E.~Arnone$^{ek,el}$,
M.~Bagheri$^{ph}$,
B.~Baret$^{cb}$,
D.~Barghini$^{el,ek}$,
M.~Battisti$^{ek,el,cb}$,
R.~Bellotti$^{ea,eb}$, 
A.A.~Belov$^{kb}$, 
M.~Bertaina$^{ek,el}$,
P.F.~Bertone$^{pf}$,
M.~Bianciotto$^{ek,el}$,
P.L.~Biermann$^{db}$,
F.~Bisconti$^{ei}$, 
C.~Blaksley$^{ft}$, 
S.~Blin-Bondil$^{cb}$, 
K.~Bolmgren$^{na}$,
S.~Briz$^{pb}$,
J.~Burton$^{pd}$,
F.~Cafagna$^{ea.eb}$, 
G.~Cambi\'e$^{ei,ej}$,
D.~Campana$^{ef}$, 
F.~Capel$^{de}$, 
R.~Caruso$^{ec,ed}$, 
M.~Casolino$^{ft,ei, ej}$,
C.~Cassardo$^{ek,el}$, 
A.~Castellina$^{ek,em}$,
K.~\v{C}ern\'{y}$^{bb}$,  
M.J.~Christl$^{pf}$, 
R.~Colalillo$^{ef,eg}$,
L.~Conti$^{en,ei}$, 
G.~Cotto$^{ek,el}$, 
H.J.~Crawford$^{pa}$, 
R.~Cremonini$^{el}$,
A.~Creusot$^{cb}$, 
A.~de Castro G\'onzalez$^{pb}$,  
C.~de la Taille$^{ca}$, 
R.~Diesing$^{pb}$,
P.~Dinaucourt$^{ca}$,
A.~Di Nola$^{eg}$,
A.~Ebersoldt$^{db}$,
T.~Ebisuzaki$^{ft}$,
J.~Eser$^{pb}$,
F.~Fenu$^{eo}$, 
S.~Ferrarese$^{ek,el}$,
G.~Filippatos$^{pc}$, 
W.W.~Finch$^{pc}$,
F. Flaminio$^{eg}$,
C.~Fornaro$^{en,ei}$,
D.~Fuehne$^{pc}$,
C.~Fuglesang$^{na}$, 
M.~Fukushima$^{fe}$, 
S.~Gadamsetty$^{ph}$,
D.~Gardiol$^{ek,em}$,
G.K.~Garipov$^{kb}$, 
E.~Gazda$^{ph}$, 
A.~Golzio$^{ek,el}$,
F.~Guarino$^{ef,eg}$, 
C.~Gu\'epin$^{pb}$,
A.~Haungs$^{db}$,
T.~Heibges$^{pc}$,,
F.~Isgr\`o$^{ef,eg}$, 
E.G.~Judd$^{pa}$, 
F.~Kajino$^{ff}$, 
I.~Kaneko$^{ft}$, 
M.~Kleifges$^{db}$,
P.A.~Klimov$^{kb}$,
I.~Kreykenbohm$^{da}$, 
J.F.~Krizmanic$^{pj}$, 
V.~Kungel$^{pc}$,  
E.~Kuznetsov$^{pd}$, 
F.~L\'opez~Mart\'inez$^{pb}$, 
D.~Mand\'{a}t$^{bc}$,
M.~Manfrin$^{ek,el}$,
A. Marcelli$^{ej}$,
L.~Marcelli$^{ei}$, 
W.~Marsza{\l}$^{ia}$, 
J.N.~Matthews$^{pg}$, 
A.~Menshikov$^{db}$,
M.~Mese$^{ef,eg}$, 
S.S.~Meyer$^{pb}$,
J.~Mimouni$^{ad}$, 
H.~Miyamoto$^{ek,el}$, 
Y.~Mizumoto$^{fi}$,
A.~Monaco$^{ea,eb}$, 
S.~Nagataki$^{ft}$, 
J.~M.~Nachtman$^{pi}$,
D.~Naumov$^{ka}$,
A.~Neronov$^{cb}$,  
T.~Nonaka$^{fe}$, 
T.~Ogawa$^{ft}$, 
S.~Ogio$^{ft}$, 
H.~Ohmori$^{ft}$, 
A.V.~Olinto$^{pb}$,
Y.~Onel$^{pi}$,
G.~Osteria$^{ef}$,  
A.N.~Otte$^{ph}$,  
A.~Pagliaro$^{eh,ed}$,  
B.~Panico$^{ef, eg}$,  
E.~Parizot$^{cb, cd}$, 
I.H.~Park$^{gb}$, 
T.~Paul$^{pe}$,
M.~Pech$^{bc}$, 
F.~Perfetto$^{ef}$,  
P.~Picozza$^{ei,ej}$, 
L.W.~Piotrowski$^{ib}$,
Z.~Plebaniak$^{ei, ej}$, 
J.~Posligua$^{pi}$,
M.~Potts$^{ph}$,
R.~Prevete$^{ef,eg}$,
G.~Pr\'ev\^ot$^{cb}$,
M.~Przybylak$^{ia}$, 
E.~Reali$^{ei, ej}$,
P.~Reardon$^{pd}$, 
M.H.~Reno$^{pi}$, 
M.~Ricci$^{ee}$, 
O.F.~Romero~Matamala$^{ph}$, 
G.~Romoli$^{ei, ej}$,
H.~Sagawa$^{fe}$, 
N.~Sakaki$^{ft}$, 
A.~Santangelo$^{dd}$, 
O.A.~Saprykin$^{kc}$,
F.~Sarazin$^{pc}$,
M.~Sato$^{fo}$, 
H.~Schieler$^{db}$,
P.~Schov\'{a}nek$^{bc}$,
V.~Scotti$^{ef,eg}$,
S.~Selmane$^{cb}$
S.A.~Sharakin$^{kb}$,
K.~Shinozaki$^{ia}$, 
S.~Stepanoff$^{ph}$,
J.F.~Soriano$^{pe}$,
J.~Szabelski$^{ia}$,
N.~Tajima$^{ft}$, 
T.~Tajima$^{ft, pn}$,
Y.~Takahashi$^{fo}$, 
M.~Takeda$^{fe}$, 
Y.~Takizawa$^{ft}$, 
C.~Tenzer$^{dd}$,
S.B.~Thomas$^{pg}$, 
L.G.~Tkachev$^{ka}$,
T.~Tomida$^{fh}$, 
S.~Toscano$^{ob}$,  
M.~Tra\"{i}che$^{aa}$,  
D.~Trofimov$^{cb,kb}$,
K.~Tsuno$^{ft}$,  
P.~Vallania$^{ek,em}$,
L.~Valore$^{ef,eg}$,
T.~M.~Venters$^{pj}$,
C.~Vigorito$^{ek,el}$, 
M.~Vrabel$^{ia}$, 
S.~Wada$^{ft}$,  
J.~Watts~Jr.$^{pd}$, 
A.~Weindl$^{db}$,
L.~Wiencke$^{pc}$, 
J.~Wilms$^{da}$,
D.~Winn$^{pm}$,
H.~Wistrand$^{pc}$,
I.V.~Yashin$^{kb}$, 
R.~Young$^{pf}$,
M.Yu.~Zotov$^{kb}$.
}
\end{sloppypar}
\vspace*{.3cm}

%%\newpage
{ \footnotesize
\noindent
% Algeria - 2 institutes
$^{aa}$ Centre for Development of Advanced Technologies (CDTA), Algiers, Algeria \\
$^{ad}$ Lab. of Math. and Sub-Atomic Phys. (LPMPS), Univ. Constantine I, Constantine, Algeria \\
% Czech Republic - 2 institutes
$^{bb}$ Joint Laboratory of Optics, Faculty of Science, Palack\'{y} University, Olomouc, Czech Republic\\
$^{bc}$ Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic\\
% France - 3 institutes  
$^{ca}$ Omega, Ecole Polytechnique, CNRS/IN2P3, Palaiseau, France\\
$^{cb}$ Universit\'e de Paris, CNRS, AstroParticule et Cosmologie, F-75013 Paris, France\\
$^{cd}$ Institut universitaire de France (IUF)\\
% Germany - 4 institutes
$^{da}$ ECAP, University of Erlangen-Nuremberg, Germany\\
$^{db}$ Karlsruhe Institute of Technology (KIT), Germany\\
$^{dd}$ Institute for Astronomy and Astrophysics, Kepler Center, University of T\"ubingen, Germany\\
$^{de}$ Max Planck Institute for Physics, Munich, Germany\\
% Italy - 15 institutes  
$^{ea}$ Istituto Nazionale di Fisica Nucleare - Sezione di Bari, Italy\\
$^{eb}$ Universita' degli Studi di Bari Aldo Moro and INFN - Sezione di Bari, Italy\\
$^{ec}$ Dipartimento di Fisica e Astronomia "Ettore Majorana", Universita' di Catania, Italy\\
$^{ed}$ Istituto Nazionale di Fisica Nucleare - Sezione di Catania, Italy\\
$^{ee}$ Istituto Nazionale di Fisica Nucleare - Laboratori Nazionali di Frascati, Italy\\
$^{ef}$ Istituto Nazionale di Fisica Nucleare - Sezione di Napoli, Italy\\
$^{eg}$ Universita' di Napoli Federico II - Dipartimento di Fisica "Ettore Pancini", Italy\\
$^{eh}$ INAF - Istituto di Astrofisica Spaziale e Fisica Cosmica di Palermo, Italy\\
$^{ei}$ Istituto Nazionale di Fisica Nucleare - Sezione di Roma Tor Vergata, Italy\\
$^{ej}$ Universita' di Roma Tor Vergata - Dipartimento di Fisica, Roma, Italy\\
$^{ek}$ Istituto Nazionale di Fisica Nucleare - Sezione di Torino, Italy\\
$^{el}$ Dipartimento di Fisica, Universita' di Torino, Italy\\
$^{em}$ Osservatorio Astrofisico di Torino, Istituto Nazionale di Astrofisica, Italy\\
$^{en}$ Uninettuno University, Rome, Italy\\
$^{eo}$ Agenzia Spaziale Italiana, Via del Politecnico, 00133, Roma, Italy\\
% Japan - 7 institutes 
$^{fe}$ Institute for Cosmic Ray Research, University of Tokyo, Kashiwa, Japan\\ 
$^{ff}$ Konan University, Kobe, Japan\\ 
$^{fh}$ Shinshu University, Nagano, Japan \\
$^{fi}$ National Astronomical Observatory, Mitaka, Japan\\ 
$^{fo}$ Hokkaido University, Sapporo, Japan \\ 
$^{fq}$ Nihon University Chiyoda, Tokyo, Japan\\ 
$^{ft}$ RIKEN, Wako, Japan\\
% Korea - 1 institute
$^{gb}$ Sungkyunkwan University, Seoul, Republic of Korea\\
% Poland - 2 institutes
$^{ia}$ National Centre for Nuclear Research, Otwock, Poland\\
$^{ib}$ Faculty of Physics, University of Warsaw, Poland\\
% Russia - 3 institutes 
$^{ka}$ Joint Institute for Nuclear Research, Dubna, Russia\\
$^{kb}$ Skobeltsyn Institute of Nuclear Physics, Lomonosov Moscow State University, Russia\\
$^{kc}$ Space Regatta Consortium, Korolev, Russia\\
% Sweden - 1 institute 
$^{na}$ KTH Royal Institute of Technology, Stockholm, Sweden\\
% Switzerland - 1 institute 
$^{ob}$ ISDC Data Centre for Astrophysics, Versoix, Switzerland\\
% USA - 12 institutes 
$^{pa}$ Space Science Laboratory, University of California, Berkeley, CA, USA\\
$^{pb}$ University of Chicago, IL, USA\\
$^{pc}$ Colorado School of Mines, Golden, CO, USA\\
$^{pd}$ University of Alabama in Huntsville, Huntsville, AL; USA\\
$^{pe}$ Lehman College, City University of New York (CUNY), NY, USA\\
$^{pf}$ NASA Marshall Space Flight Center, Huntsville, AL, USA\\
$^{pg}$ University of Utah, Salt Lake City, UT, USA\\
$^{ph}$ Georgia Institute of Technology, USA\\
$^{pi}$ University of Iowa, Iowa City, IA, USA\\
$^{pj}$ NASA Goddard Space Flight Center, Greenbelt, MD, USA\\
$^{pm}$ Fairfield University, Fairfield, CT, USA\\
$^{pn}$ Department of Physics and Astronomy, University of California, Irvine \\
}


==> JEM-EUSO_Authors_July2023_final.tex <==
\newpage
{\Large\bf Full Authors list: The JEM-EUSO Collaboration\\}
%{\scriptsize (author-list as of July 15th, 2023 with reorganized affiliations)} \hspace{0.6cm}
%{\scriptsize (version  \today{} \currenttime{})}
%\vspace*{0.5cm}

\begin{sloppypar}
{\small \noindent
S.~Abe$^{ff}$, 
J.H.~Adams Jr.$^{ld}$, 
D.~Allard$^{cb}$,
P.~Alldredge$^{ld}$,
R.~Aloisio$^{ep}$,
L.~Anchordoqui$^{le}$,
A.~Anzalone$^{ed,eh}$, 
E.~Arnone$^{ek,el}$,
M.~Bagheri$^{lh}$,
B.~Baret$^{cb}$,
D.~Barghini$^{ek,el}$,
M.~Battisti$^{cb,ek,el}$,
R.~Bellotti$^{ea,eb}$, 
A.A.~Belov$^{ib}$, 
M.~Bertaina$^{ek,el}$,
P.F.~Bertone$^{lf}$,
M.~Bianciotto$^{ek,el}$,
F.~Bisconti$^{ei}$, 
C.~Blaksley$^{fg}$, 
S.~Blin-Bondil$^{cb}$, 
K.~Bolmgren$^{ja}$,
S.~Briz$^{lb}$,
J.~Burton$^{ld}$,
F.~Cafagna$^{ea.eb}$, 
G.~Cambi\'e$^{ei,ej}$,
D.~Campana$^{ef}$, 
F.~Capel$^{db}$, 
R.~Caruso$^{ec,ed}$, 
M.~Casolino$^{ei,ej,fg}$,
C.~Cassardo$^{ek,el}$, 
A.~Castellina$^{ek,em}$,
K.~\v{C}ern\'{y}$^{ba}$,  
M.J.~Christl$^{lf}$, 
R.~Colalillo$^{ef,eg}$,
L.~Conti$^{ei,en}$, 
G.~Cotto$^{ek,el}$, 
H.J.~Crawford$^{la}$, 
R.~Cremonini$^{el}$,
A.~Creusot$^{cb}$,
A.~Cummings$^{lm}$,
A.~de Castro G\'onzalez$^{lb}$,  
C.~de la Taille$^{ca}$, 
R.~Diesing$^{lb}$,
P.~Dinaucourt$^{ca}$,
A.~Di Nola$^{eg}$,
T.~Ebisuzaki$^{fg}$,
J.~Eser$^{lb}$,
F.~Fenu$^{eo}$, 
S.~Ferrarese$^{ek,el}$,
G.~Filippatos$^{lc}$, 
W.W.~Finch$^{lc}$,
F. Flaminio$^{eg}$,
C.~Fornaro$^{ei,en}$,
D.~Fuehne$^{lc}$,
C.~Fuglesang$^{ja}$, 
M.~Fukushima$^{fa}$, 
S.~Gadamsetty$^{lh}$,
D.~Gardiol$^{ek,em}$,
G.K.~Garipov$^{ib}$, 
E.~Gazda$^{lh}$, 
A.~Golzio$^{ek,el}$,
F.~Guarino$^{ef,eg}$, 
C.~Gu\'epin$^{lb}$,
A.~Haungs$^{da}$,
T.~Heibges$^{lc}$,
F.~Isgr\`o$^{ef,eg}$, 
E.G.~Judd$^{la}$, 
F.~Kajino$^{fb}$, 
I.~Kaneko$^{fg}$,
S.-W.~Kim$^{ga}$,
P.A.~Klimov$^{ib}$,
J.F.~Krizmanic$^{lj}$, 
V.~Kungel$^{lc}$,  
E.~Kuznetsov$^{ld}$, 
F.~L\'opez~Mart\'inez$^{lb}$, 
D.~Mand\'{a}t$^{bb}$,
M.~Manfrin$^{ek,el}$,
A. Marcelli$^{ej}$,
L.~Marcelli$^{ei}$, 
W.~Marsza{\l}$^{ha}$, 
J.N.~Matthews$^{lg}$, 
M.~Mese$^{ef,eg}$, 
S.S.~Meyer$^{lb}$,
J.~Mimouni$^{ab}$, 
H.~Miyamoto$^{ek,el}$, 
Y.~Mizumoto$^{fd}$,
A.~Monaco$^{ea,eb}$, 
S.~Nagataki$^{fg}$, 
J.M.~Nachtman$^{li}$,
D.~Naumov$^{ia}$,
A.~Neronov$^{cb}$,  
T.~Nonaka$^{fa}$, 
T.~Ogawa$^{fg}$, 
S.~Ogio$^{fg}$, 
H.~Ohmori$^{fg}$, 
A.V.~Olinto$^{lb}$,
Y.~Onel$^{li}$,
G.~Osteria$^{ef}$,  
A.N.~Otte$^{lh}$,  
A.~Pagliaro$^{ed,eh}$,  
B.~Panico$^{ef,eg}$,  
E.~Parizot$^{cb,cc}$, 
I.H.~Park$^{gb}$, 
T.~Paul$^{le}$,
M.~Pech$^{bb}$, 
F.~Perfetto$^{ef}$,  
P.~Picozza$^{ei,ej}$, 
L.W.~Piotrowski$^{hb}$,
Z.~Plebaniak$^{ei,ej}$, 
J.~Posligua$^{li}$,
M.~Potts$^{lh}$,
R.~Prevete$^{ef,eg}$,
G.~Pr\'ev\^ot$^{cb}$,
M.~Przybylak$^{ha}$, 
E.~Reali$^{ei, ej}$,
P.~Reardon$^{ld}$, 
M.H.~Reno$^{li}$, 
M.~Ricci$^{ee}$, 
O.F.~Romero~Matamala$^{lh}$, 
G.~Romoli$^{ei, ej}$,
H.~Sagawa$^{fa}$, 
N.~Sakaki$^{fg}$, 
O.A.~Saprykin$^{ic}$,
F.~Sarazin$^{lc}$,
M.~Sato$^{fe}$, 
P.~Schov\'{a}nek$^{bb}$,
V.~Scotti$^{ef,eg}$,
S.~Selmane$^{cb}$,
S.A.~Sharakin$^{ib}$,
K.~Shinozaki$^{ha}$, 
S.~Stepanoff$^{lh}$,
J.F.~Soriano$^{le}$,
J.~Szabelski$^{ha}$,
N.~Tajima$^{fg}$, 
T.~Tajima$^{fg, ll}$,
Y.~Takahashi$^{fe}$, 
M.~Takeda$^{fa}$, 
Y.~Takizawa$^{fg}$, 
S.B.~Thomas$^{lg}$, 
L.G.~Tkachev$^{ia}$,
T.~Tomida$^{fc}$, 
S.~Toscano$^{ka}$,  
M.~Tra\"{i}che$^{aa}$,  
D.~Trofimov$^{cb,ib}$,
K.~Tsuno$^{fg}$,  
P.~Vallania$^{ek,em}$,
L.~Valore$^{ef,eg}$,
T.M.~Venters$^{lj}$,
C.~Vigorito$^{ek,el}$, 
M.~Vrabel$^{ha}$, 
S.~Wada$^{fg}$,  
J.~Watts~Jr.$^{ld}$, 
L.~Wiencke$^{lc}$, 
D.~Winn$^{lk}$,
H.~Wistrand$^{lc}$,
I.V.~Yashin$^{ib}$, 
R.~Young$^{lf}$,
M.Yu.~Zotov$^{ib}$.
}
\end{sloppypar}
\vspace*{.3cm}

%%\newpage
{ \footnotesize
\noindent
% Algeria - 2 institutes
$^{aa}$ Centre for Development of Advanced Technologies (CDTA), Algiers, Algeria \\
$^{ab}$ Lab. of Math. and Sub-Atomic Phys. (LPMPS), Univ. Constantine I, Constantine, Algeria \\
% Czech Republic - 2 institutes
$^{ba}$ Joint Laboratory of Optics, Faculty of Science, Palack\'{y} University, Olomouc, Czech Republic\\
$^{bb}$ Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic\\
% France - 3 institutes  
$^{ca}$ Omega, Ecole Polytechnique, CNRS/IN2P3, Palaiseau, France\\
$^{cb}$ Universit\'e de Paris, CNRS, AstroParticule et Cosmologie, F-75013 Paris, France\\
$^{cc}$ Institut Universitaire de France (IUF), France\\
% Germany - 2 institutes
$^{da}$ Karlsruhe Institute of Technology (KIT), Germany\\
$^{db}$ Max Planck Institute for Physics, Munich, Germany\\
% Italy - 16 institutes  
$^{ea}$ Istituto Nazionale di Fisica Nucleare - Sezione di Bari, Italy\\
$^{eb}$ Universit\`a degli Studi di Bari Aldo Moro, Italy\\
$^{ec}$ Dipartimento di Fisica e Astronomia "Ettore Majorana", Universit\`a di Catania, Italy\\
$^{ed}$ Istituto Nazionale di Fisica Nucleare - Sezione di Catania, Italy\\
$^{ee}$ Istituto Nazionale di Fisica Nucleare - Laboratori Nazionali di Frascati, Italy\\
$^{ef}$ Istituto Nazionale di Fisica Nucleare - Sezione di Napoli, Italy\\
$^{eg}$ Universit\`a di Napoli Federico II - Dipartimento di Fisica "Ettore Pancini", Italy\\
$^{eh}$ INAF - Istituto di Astrofisica Spaziale e Fisica Cosmica di Palermo, Italy\\
$^{ei}$ Istituto Nazionale di Fisica Nucleare - Sezione di Roma Tor Vergata, Italy\\
$^{ej}$ Universit\`a di Roma Tor Vergata - Dipartimento di Fisica, Roma, Italy\\
$^{ek}$ Istituto Nazionale di Fisica Nucleare - Sezione di Torino, Italy\\
$^{el}$ Dipartimento di Fisica, Universit\`a di Torino, Italy\\
$^{em}$ Osservatorio Astrofisico di Torino, Istituto Nazionale di Astrofisica, Italy\\
$^{en}$ Uninettuno University, Rome, Italy\\
$^{eo}$ Agenzia Spaziale Italiana, Via del Politecnico, 00133, Roma, Italy\\
$^{ep}$ Gran Sasso Science Institute, L'Aquila, Italy\\
% Japan - 7 institutes 
$^{fa}$ Institute for Cosmic Ray Research, University of Tokyo, Kashiwa, Japan\\ 
$^{fb}$ Konan University, Kobe, Japan\\ 
$^{fc}$ Shinshu University, Nagano, Japan \\
$^{fd}$ National Astronomical Observatory, Mitaka, Japan\\ 
$^{fe}$ Hokkaido University, Sapporo, Japan \\ 
$^{ff}$ Nihon University Chiyoda, Tokyo, Japan\\ 
$^{fg}$ RIKEN, Wako, Japan\\
% Korea - 2 institutes
$^{ga}$ Korea Astronomy and Space Science Institute\\
$^{gb}$ Sungkyunkwan University, Seoul, Republic of Korea\\
% Poland - 2 institutes
$^{ha}$ National Centre for Nuclear Research, Otwock, Poland\\
$^{hb}$ Faculty of Physics, University of Warsaw, Poland\\
% Russia - 3 institutes 
$^{ia}$ Joint Institute for Nuclear Research, Dubna, Russia\\
$^{ib}$ Skobeltsyn Institute of Nuclear Physics, Lomonosov Moscow State University, Russia\\
$^{ic}$ Space Regatta Consortium, Korolev, Russia\\
% Sweden - 1 institute 
$^{ja}$ KTH Royal Institute of Technology, Stockholm, Sweden\\
% Switzerland - 1 institute 
$^{ka}$ ISDC Data Centre for Astrophysics, Versoix, Switzerland\\
% USA - 13 institutes 
$^{la}$ Space Science Laboratory, University of California, Berkeley, CA, USA\\
$^{lb}$ University of Chicago, IL, USA\\
$^{lc}$ Colorado School of Mines, Golden, CO, USA\\
$^{ld}$ University of Alabama in Huntsville, Huntsville, AL, USA\\
$^{le}$ Lehman College, City University of New York (CUNY), NY, USA\\
$^{lf}$ NASA Marshall Space Flight Center, Huntsville, AL, USA\\
$^{lg}$ University of Utah, Salt Lake City, UT, USA\\
$^{lh}$ Georgia Institute of Technology, USA\\
$^{li}$ University of Iowa, Iowa City, IA, USA\\
$^{lj}$ NASA Goddard Space Flight Center, Greenbelt, MD, USA\\
$^{lk}$ Fairfield University, Fairfield, CT, USA\\
$^{ll}$ Department of Physics and Astronomy, University of California, Irvine, USA \\
$^{lm}$ Pennsylvania State University, PA, USA \\
}


